Multivariate Time Series Cleaning under Speed Constraints

Errors are common in time series due to unreliable sensor measurements. Existing methods focus on univariate data but do not utilize the correlation between dimensions. Cleaning each dimension separately may lead to a less accurate result, as some errors can only be identified in the multivariate case. We also point out that the widely used minimum change principle is not always the best choice. Instead, we try to change the smallest number of data to avoid a significant change in the data distribution. In this paper, we propose MTCSC, the constraint-based method for cleaning multivariate time series. We formalize the repair problem, propose a linear-time method to employ online computing, and improve it by exploiting data trends. We also support adaptive speed constraint capturing. We analyze the properties of our proposals and compare them with SOTA methods in terms of effectiveness, efficiency versus error rates, data sizes, and applications such as classification. Experiments on real datasets show that MTCSC can have higher repair accuracy with less time consumption. Interestingly, it can be effective even when there are only weak or no correlations between the dimensions.

==> tex/revision.tex <==
% !TEX root = ../speed.tex

% revision --------------------------------------------
\makeatletter
\newenvironment{question}[1][Q]{\par
\addvspace{6pt plus 6pt}% \vspace{-\topsep}% remove the space after the theorem
%\pushQED{\qed}%
  %\fontsize{10pt}{1.5em}
  \normalfont \partopsep=\z@skip \topsep=\z@skip
  \trivlist
  \item[\hskip\labelsep
        \bfseries
    #1\@addpunct{:}]\ignorespaces
    \itshape\color{blue}
}{%
%  \popQED
\endtrivlist\@endpefalse
%  \addvspace{6pt plus 6pt} % some space after
}
\newenvironment{reply}[1][Reply]{\par
%\addvspace{3pt plus 3pt}% \vspace{-\topsep}% remove the space after the theorem
  \pushQED{\qed}%
%  \fontsize{10pt}{1.5em}
  \normalfont \partopsep=\z@skip \topsep=\z@skip
  \trivlist
  \item[\hskip\labelsep
        \scshape
    #1\@addpunct{:}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
%  \addvspace{6pt plus 6pt} % some space after
}
\makeatother
%\newenvironment{revised2}{\color{blue}}{}
%\newenvironment{revised4}{\color{red}}{}
%\newenvironment{revised5}{\color{magenta}}{}
%\newenvironment{revised5}{\color{cadmiumgreen}}{}

%\twocolumn[
\begin{center}
\textsf{Multivariate Time Series Cleaning under Speed Constraints (Original Paper ID: 373, Shepherd Submission ID: 492)}
\end{center}
%]


%Firstly, we thank the reviewers for insightful comments and constructive suggestions towards an improvement of our submission. Below is the summary of major changes in the revised manuscript. 
%We list the detailed responses to the comments from each reviewer.


%===================================
\section*{To Meta Reviewer}

Thank you very much for your comments.
We have addressed the reviewers' concerns and revision requests in the revised manuscript.
Due to the space limit, we remove some unconcerned parts in the original version.
Please find our response as follows.

\begin{question}[C1]
Better justification of why the minimum fix principle and speed constraints are relevant to the problem at hand.
\end{question}

\begin{reply}
(1) Following the minimum fix principle can better reduce the number of correct points that are changed and achieve more accurate results.
See R1.O1 for more detailed replies.
(2) Speed constraint is valid in theory, applicable in practice and accommodates the non-stationary property of time series. 
See R1.O2(1) for more detailed replies.
\end{reply}

\begin{question}[C2]
Justification of technical choices, and why magnitude of change is not considered.
\end{question}

\begin{reply}
(1) The optimization solver (like Gurobi) is not only applicable to univariate input, but can also solve multivariate input directly. For why and how to use the optimization solver, see R1.O4 (1) for more detailed replies.
(2) The optimization solver can lead to a global optimal solution, but it costs too much time.
Therefore, we propose \textsf{MTCSC-G} (DP algorithm) to determine which data points need to be fixed to improve efficiency.
For why to propose DP algorithm in Section \ref{sect:global-dp} and how each point and repair value is chosen, see R1.O4 (2) for more detailed replies.
(3) In contrast to previous work, we follow the minimum fix principle to minimize the number of points changed from the original time series and obtain more accurate repairs.
Therefore, we do not consider the magnitude of change as the object in the optimization problem.
For why magnitude of change is not considered, see R1.O4 (3) for more detailed replies.
\end{reply}

\begin{question}[C3]
Why are only adjacent points used in the repair value computation?
\end{question}

\begin{reply}
Proposition \ref{the:pre-range} and Proposition \ref{the:post-range} state that considering the nearest preceding point and succeeding point is sufficient to determine the range of possible repairs, respectively.
See R1.O5 for more detailed replies.
\end{reply}

\begin{question}[C4]
More details and justification for the selected baselines.
\end{question}

\begin{reply}
\textsf{SCREEN} and \textsf{SpeedAcc} use the univariate speed constraint and follow the widely used minimum change principle.
They are selected to verify the validity of the proposed minimum fix principle.
We want to conduct a comprehensive comparison with these competing baselines of different types (listed in Table \ref{table:baseline}) in different scenarios to validate the effectiveness and efficiency of our proposal.
See R1.O8 for more detailed replies.
\end{reply}

\begin{question}[C5]
The implementation of an error guarantee for the adaptive speed version w.r.t. to the parameters b, theta, w, and beta.
\end{question}

\begin{reply}
As shown in formulas (\ref{equation:global}) and (\ref{equation:local}), our work aims to minimize the number of points changed from the original time series
However, similar to the statements in Section \ref{sect:stream}, we do not have a theoretical upper bound for \textsf{MTCSC-A} compared to \textsf{MTCSC-C}.
See R4.O2 for more detailed replies.
\end{reply}

\begin{question}[C6]
How are the algorithms scaling with the number of dimensions.
\end{question}

\begin{reply}
%Although the time required to calculate the distance is slightly larger for a large number of dimensions is slightly larger, it is still applicable.
%As shown in Figure \ref{exp:drate-together}(d), \textsf{MTCSC} finishes in about 10 ms, just a bit slower than its Uni version.
%See R4.O5 for more detailed replies.
We add an experiment in Section \ref{sect:exp-dimension} under the "together" pattern over all the proposed methods (\textsf{MTCSC-G}, \textsf{MTCSC-L} and \textsf{MTCSC-C}) and analyze the results of varying dimensions.
See R4.O5 for more detailed replies.
\end{reply}

%----------------------------------
\section*{To Reviewer 1}
Thank you very much for reading our paper carefully. 
Below is our response to your comments.
%{Accept with Shepherding}

\begin{question}[O1]
O1: The minimum fix principle needs to be better justified as to why this is the correct and ``best'' philosophy to take.
\end{question}

\begin{reply}
%Errors are rare in the real world [need a citation].
The minimum change principle refers to the minimum sum of changes between the repaired value and the original value.
Although the original correct data has been modified as little as possible, a certain part of the correct data is still changed, which is confirmed by the experimental results in Figures \ref{exp:temp-drate}(d) and \ref{exp:temp-size}(d).
In turn, we use the minimum fix principle, i.e. the number of modified points is minimized.
As shown in Figures \ref{exp:temp-drate}(d) and \ref{exp:temp-size}(d), the number of points modified by \textsf{MTCSC} is relatively similar to the number of manually injected errors.
Thus, the proposed \textsf{MTCSC} can accurately identify error points and achieve better results.

We add ``since a certain portion of originally clean data is still changed'' in the first paragraph of Section \ref{sect:solution}, after ``Moreover, we do not follow ...''.

We add the justification in Section \ref{sect:uni-drate} as follows: 
As shown in Figures \ref{exp:temp-drate}(c) and (d),
we find that \textsf{SCREEN}, \textsf{SpeedAcc}, \textsf{LsGreedy}, and \textsf{HTD},
which are based on the minimum change principle, modify many more points than our proposed \textsf{MTCSC}, which is based on the minimum fix principle, resulting in an even larger repair distance.
Moreover, the number of points modified by \textsf{MTCSC} is relatively similar to the number of manually injected errors.
\end{reply}

\begin{question}[O2]
O2: The paper presents challenges for multi-dimensional time series cleaning but does not adequately justify why speed constraints, in particular, are the right choice. 
Given the need to adaptively update these constraints upon change detection, it seems that this would incur a costly overhead.
\end{question}

\begin{reply}
In the following, we first explain that speed constraints are the right choice and then show that the additional costs are worthwhile.

(1) The justification for the use of speed constraints is as follows:
(a) Speed constraint is valid in theory.
As stated in the paragraphs after Definition \ref{definition:speed-constraint} in Section \ref{sect:constraint}, speed constraints are often useful in real-world scenarios and the ``jump'' of values in time series data within a short time period is usually limited.
(b) Speed constraint is applicable in practice.
It supports online cleaning and takes less time while maintaining relatively good repair accuracy.
Time series is naturally infinite.
An online method can better meet these requirements.
(c) Speed constraint can be efficiently captured dynamically, which accommodates the non-stationary property of time series.
We add reasons (b) and (c) into Section \ref{sect:constraint} to show that using speed constraints is the right choice.

(2) Adaptive updating of speed constraints would take more time, but it is worth doing:
(a) It is known that an accurate speed constraint is crucial for constraint-based methods such as \cite{DBLP:conf/sigmod/SongZWY15, taylor2019dynamic}.
The maximum speed people can reach depends on their mode of transportation.
As shown in Section \ref{sect:transportation}, according to common sense, the speed constraint corresponding to walking, running and cycling are quite different.
We also expect to adaptively determine proper speed constraints in fileds without sufficient domain knowledge.
(b) We apologize for using the same term ``window size'' for two different variables in this paper, which can lead to confusion.
%We provide the dedicated algorithm, i.e. Algorithm 5: \textsf{MTCSC-A}($\boldsymbol{\mathit{x}}, \mathit{s}$, $\mathit{b}$, $\tau$, $\mathit{m}$, $\beta$), in Section \ref{sect:adaptive-speed} to show the procedure of the adaptive method.
%The time complexity is $O(\mathit{m}+\mathit{b})+O(\mathit{w}^{2}n)$, where $m$ is the adaptive speed monitoring interval, $b$ is the bucket number, $w$ is the point window size, and $n$ is the length of the time series.
%Compared to the time complexity $O(\mathit{w}^{2}n)$ of Algorithm \ref{alg:cluster} presented in Section \ref{sect:repair-via-cluster}, we know that the additional cost of the adaptive method is not significant.
We change the second ``window size'' to ``monitoring interval'' in the revised version.
We provide the dedicated algorithm, i.e. Algorithm \ref{alg:adaptive}: \textsf{AdaptiveSpeed}($\boldsymbol{\mathit{x}}_p, \boldsymbol{\mathit{x}}_k, \mathit{s}$, $\mathit{b}$, $\tau$, $\mathit{m}$, $\beta$, $\mathit{W}_1$, $\mathit{W}_2$), in Section \ref{sect:adaptive-speed} to show the core procedure of the online cleaning method \textsf{MTCST-A} with adaptive speed.
The time complexity of Algorithm \ref{alg:adaptive} is $O(\mathit{D}+\mathit{b}+\mathit{m})$. 
\textsf{MTCSC-A} is formed by inserting Algorithm \ref{alg:adaptive} through ``$\mathit{s}$ = \textsf{AdaptiveSpeed}($\boldsymbol{\mathit{x}}_{k-1}, \boldsymbol{\mathit{x}}_k, \mathit{s}$, $\mathit{b}$, $\tau$, $\mathit{m}$, $\beta$, $\mathit{W}_1$, $\mathit{W}_2$)'' between the 3rd and 4th lines of Algorithm \ref{alg:cluster}.
Overall, the time complexity of \textsf{MTCSC-A} is $O((\mathit{D}+\mathit{b}+\mathit{m}+\mathit{w}^{2}D+2D)*n)$, where $m$ is the adaptive speed monitoring interval, $b$ is the bucket number, $w$ is the point window size, and $n$ is the length of the time series.
Compared to the time complexity $O((\mathit{w}^{2}D+2D)*n)$ of Algorithm \ref{alg:cluster} presented in Section \ref{sect:repair-via-cluster}, we know that the additional cost of the adaptive method is not significant.
\end{reply}

\begin{question}[O3]
O3: What is the cost to identify violations using speed constraints? The paper seems to assume violations are readily available.
\end{question}

\begin{reply}
In order to separate out the detection time instead of embed it into the overall algorithm, we make a deeper analysis of all the proposed algorithms in the revised version and report both the detection time complexity and overall time complexity. 
The judgment procedure \textsf{satisfy}$(\boldsymbol{\mathit{x}}_i, \boldsymbol{\mathit{x}}_j)$ costs $O(D)$ time where D is the dimension of time series. Hence:
(1) Algorithm \ref{alg:global} (\textsf{MTCSC-G}) outputs the \emph{FixList} that contains all the points need to be fixed, which is in fact the detection of violations and the detection time is $O(Dn^2)$. 
The overall time complexity is $O(Dn^2) + O(fD) = O(Dn^2)$ where $f$ is the number of all the points need to be fixed and the worst-case scenario is $f = n/2$.
(2) Algorithm \ref{alg:local} (\textsf{MTCSC-L}) detects the violation for each data point in Line 2 and the time cost is $O(D)$. 
Thus, the total detection time complexity is $O(Dn)$ and the overall time complexity is $O(Dn) + O(wDn) = O(wDn)$.
(3) We apologize for the typo in the previous version of Algorithm \ref{alg:cluster}. 
\textsf{MTCSC-C} misses a judgment condition ``if !(\textsf{satisfy}$(\boldsymbol{\mathit{x}}'_{k-1}, x_{k})$ and \textsf{satisfy}$(\boldsymbol{\mathit{x}}_k, \boldsymbol{\mathit{x}}_i)$''. 
For each data point, we need to build the clusters first and then detect the violations. 
Thus, the total detection time complexity is $O(w^2Dn) + O(2Dn) = O(w^2Dn)$ and the overall time complexity is $O(w^2Dn)$
\end{reply}

\begin{question}[O4]
O4: Parts of the methodology need more clarification and justification.
In Sec. 2.2, there is a good formalization of the problem. However, the optimization solver seems to assume a univariate input and states solvers like Gurobi can be used directly. 
This is not clear why, and a description and justification of this proposed approach needs to be given. 

This continues in follow-on sections, e.g., Sec. 2.2.2 where the DP algorithm is described. 
However, more explanation is needed to justify how each point and repair value is chosen. 

It seems odd to me that the magnitude of change is not considered in the optimization problem, since there are a range of values that can be proposed as a repair and how an ``optimal'' one is chosen is not explained.
\end{question}

\begin{reply}
(1) In Section \ref{sect:global}, the optimization solver (like Gurobi) is not only applicable to univariate input, but can also solve multivariate input directly.
For univariate inputs, the highest degree of the constraint part is 1, hence it is called MILP.
For multivariate inputs, the highest degree of the constraint part is 2, so it is called MIQP.
Example \ref{example:optimization-solver} shows the result of Gurobi on the two-dimensional data as input.
We add more explanations at the end of Section \ref{sect:global-solver} to justify how each points and repair values are selected:
Once the input time series has been converted to the constraint type, according to the formulas (\ref{equation:global-max}) and (\ref{equation:global-repair}), where M is set to 1000, it can be fed directly into an existing optimization solver.
The output of the solver is the repair values of each data points and can be the ``optimal'' solution under our problem definition.

%(2)Due to the limitation of length, this article provides a brief explanation of the selection of repair values in Example \ref{example:global-dp}, which states ``We use the `clean' points (considered clean by Algorithm 1) closed to the detected points on both sides for repair.'' on line 377.
%Similialy, due to the limitation of length, this paper did not explain the correctness of selecting the points that need to be repaired. The explanation is as follows:
%
%%The global optimal problem is to find a repair that satisfies the speed constraint on the overall data pairwise, while minimizing the number of repaired points. The DP algorithm in section 2.2.2 is an extension of the longest increasing subsequence problem(LIS), which is to find the longest continuously increasing subsequence in the overall sequence. Therefore, points that are not within the subsequence do not greater than their preceding points or less than their succeeding points. This is equivalent to an increasing constraint, which can be transformed into a speed constraint. At the same time, the subsequence is the longest, which means that only these points that are not in the subsequence need to be modified to satisfy the increasing constraint, and the entire sequence can be continuously increasing. This can be transformed into the point with the least modification. For example, a sequence is $[10,22,9,33,21,50,41,60,80]$, the longest increasing subsequence is $[10,22,33,50,60,80]$, and the remaining points are $[9,21,41]$. If these points are modified to correspond to $[27, 41.5, 55]$, and the new sequence is $[10, 22, 27, 33, 41.5, 50, 55, 60, 80]$, then the longest increasing subsequence of the sequence is itself, and the number of modified points is also the smallest.
%
%The global optimization problem is to repair the data, satisfying the pairwise speed constraint while minimizing repaired points.
%The DP algorithm in section \ref{sect:global-dp} extends the longest increasing subsequence problem(LIS), ensuring points inside the subsequence adhere to the increasing constraint.
%By modifying only these points outside the subsequence, the entire sequence remains continuously increasing.
%For example, in [10,22,9,33,21,50,41,60,80], modifying [9,21,41] to [27, 41.5, 55] results in [10, 22, 27, 33, 41.5, 50, 55, 60, 80] adhere to the increasing constraint and minimal modifications.

(2) Due to the limit of space, we only briefly explained how to select repair values for the DP algorithm in Example \ref{example:global-dp}.
As suggested, we modify the content and add further explanation in Section \ref{sect:global-dp} as follows:
The optimization solver can lead to a global optimal solution, but it costs too much time.
Therefore, we propose Algorithm \ref{alg:global} to determine which data points need to be fixed to improve efficiency.
It is an extension of the longest increasing subsequence problem (LIS) \cite{schensted1961longest}.
Our goal is to find the longest subsequence in the entire time series that satisfies the given speed constraint, which is equivalent to the LIS problem of finding the longest increasing subsequence.
Once it is found (i.e. \emph{CleanList}), the data points that are not included in this list must be repaired and are guaranteed to be the least modified (i.e. minimum fix).

Also, at the end of the Section \ref{sect:global-dp}, we add the way to select the repair values as follows:
Finally, for each point in \emph{FixList}, we can easily find the nearest preceding point $\boldsymbol{\mathit{x}}_p$ and the nearest succeeding point $\boldsymbol{\mathit{x}}_m$ in \emph{CleanList}.
The interpolation of these two points according to the formula \ref{equation:local-stream} is used as the final repair result.
The correctness can be verified in Proposition \ref{the:pre-range} and Proposition \ref{the:post-range} in Section \ref{sect:stream}. 

%(3) There is indeed a range of values that can be proposed as a repair, but our calculation of repair values using only adjacent points is based on the assumption that the speed between adjacent points will not suddenly change.
%Therefore, it is believed that the adjacent two points of the point to be repaired can more accurately represent the speed of the point to be repaired, thereby obtaining a more likely repair value.
(3) As mentioned before, in contrast to previous work, we follow the minimum fix principle to minimize the number of points changed from the original time series and obtain more accurate repairs.
Therefore, we do not consider the magnitude of change as the object in the optimization problem.
However, the vanilla output of optimization solvers can be the ``optimal'' solution under our problem definition, but still has room for improvement w.r.t. the magnitude of change.
Referring to R1.O5, we finally use adjacent points to generate the solution. 
The experimental results (Figure \ref{exp:stock}) show that such a heuristic method can achieve better accuracy.
To remove the ambiguity, we delete the word ``optimal'' in line 496 of the original draft.
Moreover, we state the limitation of not considering the magnitude of changes at the end of Section \ref{sect:global-solver}.
\end{reply}

\begin{question}[O5]
O5: For a given window w, why are only the adjacent points used during the computation of a repair value? 
Given the motivation of the paper to include correlations among multi-variate time series, why not make the scope of the repaired value larger than adjacent values?
\end{question}

\begin{reply}
%(1) This is based on the assumption that the speed between adjacent points will not suddenly change. 
%Therefore, it is believed that the adjacent two points of the point to be repaired can more accurately represent the speed of the point to be repaired, thereby obtaining a more likely repair value.
%
%(2) The connection between dimensions relies on speed constraints, and adjacent points refer to adjacent timestamps, not adjacent dimensions at a particular moment. The examples in this paper are all two-dimensional data. The following will give examples of four-dimensional data to better explain the principles of the algorithm.
In Section \ref{sect:global} and \ref{sect:local}, we formalize the global and local optimal problem, respectively.
Using the formulas (\ref{equation:global-repair}) and (\ref{equation:local}), we can see that the scope of repaired values (candidates) is selected from a large range.
Finally, the outputs of the solvers are used as repaired values.

For the streaming environment, however, we propose two propositions.
Proposition \ref{the:pre-range} states that considering the last $\boldsymbol{\mathit{x}}'_{k-1}$ is sufficient to determine the range of possible repairs for $\boldsymbol{\mathit{x}}'_{k}$.
Proposition \ref{the:post-range} shows that the consideration of the nearest succeeding point is sufficient to determine the range of possible repairs.
Combined with the assumption that the sequence of speed changes is stationary for a short period of time \cite{DBLP:journals/vldb/WangZSW24}, we use the idea of interpolation and use only the adjacent points (\textsf{MTCSC-C} chooses a more appropriate succeeding point via cluster) and provide a local solution.
The experimental results in Figures \ref{exp:stock}-\ref{exp:adaptive-speed} show the effectiveness of the proposed solutions.
We add the summary of this justification in Section \ref{sect:candidate-range} of the revised version.
%
%In addition, the correlation between the dimensions is taken into account by the speed constraints defined in the multivariate case (shown in Section \ref{sect:constraint}).
%Examples in this paper are two-dimensional data so that the reader can better understand our proposal.
\end{reply}

\begin{question}[O6]
O6: For a fixed w, is there an option to adjust the threshold $\tau$? Similarly, for a fixed $\tau$, can we adaptively adjust w to better improve accuracy?
\end{question}

\begin{reply}
Unfortunately, in the current version, we consider all these parameters as hyper-parameters and set them in advance (by grid search for each dataset).
According to Figures \ref{fig:KL}(b) and \ref{exp:sensitivity}(b), determining the threshold value $\tau$ is relatively simple.
In Figure \ref{fig:KL}(b), there is a clear peak in the KL divergence when the speed changes, and in Figure \ref{exp:sensitivity}(b), the threshold range for achieving good repair results is still relatively large.

In contrast, the dynamic adjustment of window size $\mathit{w}$ is non-trivial, which refers to \textsf{SCREEN}\cite{DBLP:conf/sigmod/SongZWY15}, and we need further investigation.

However, adaptively adjusting the threshold $\tau$ (under a fixed w) and window size w (under a fixed $\tau$) is a good idea and will further enhance the practicality of our proposed algorithm, which we will investigate in future work.
\end{reply}

\begin{question}[O7]
O7: Instead of referring to [32], please describe how methodology of how errors were injected in the evaluation.
\end{question}

\begin{reply}
As suggested, we describe how methodology of how errors were injected in the evaluation instead of just referring to \cite{DBLP:conf/sigmod/SongZWY15} and add the following paragraph in \ref{sect:datasets}:
%
Errors are injected by randomly replacing the values of some data points in a given dimension.
For each replaced data point, it takes a random value between the minimum and maximum values in the dataset.

In addition, the way of how to inject errors with different patterns and applications is re-organized in Section \ref{sect:error-pattern} and \ref{sect:application}.
\end{reply}

\begin{question}[O8]
O8: While I appreciate the comparison to univariate time series, how is the proposed work compared to SCREEN [32], which itself is using speed constraints?
Similarly, HoloClean is not meant to be a time series data cleaning method, so how is this applied?
A discussion on how and why each of these methods were chosen would certainly be helpful here. (Sec. 5.2).
\end{question}

\begin{reply}
%(1) In the baselines, \textsf{SCREEN} and \textsf{SpeedAcc} both use speed constraint, but these two methods are based on the minimum change principle, while the method proposed in this paper is based on the minimum fix principle.
%From Figures \ref{exp:temp-drate} and \ref{exp:temp-size}, it can be seen that the repair performance of \textsf{MTCSC-Uni} in this paper is significantly better than other benchmark algorithms, including \textsf{SCREEN}, while the time consumption does not significantly increase.
(1) \textsf{SCREEN} \cite{DBLP:conf/sigmod/SongZWY15} states that it is the first constraint-based study on univariate stream data cleaning.
The goal is to find a repaired sequence that satisfies the speed constraints and minimally differs from the original sequence.
In contrast, we define the speed constraints in the multivariate case and aim to minimize the number of points changed from the original time series.
Moreover, by considering the data distribution in the current window, the proposed \textsf{MTCSC-C} method can also fix the small errors that actually meet the speed constraints.
Figures \ref{exp:temp-drate} and \ref{exp:temp-size} show that, \textsf{MTCSC-C} performs far better than other baselines, including \textsf{SCREEN}, while the time cost does not increase significantly.

%(2) \textsf{Holoclean} is indeed not a time series data cleaning method, it is proposed for relational databases.
%Thus, we change time series data into relational data, with timestamps and the values of each dimension treated as attributes.
%The denail constraint of \textsf{Holoclean} is set as a speed constraint after the quantization of data for each dimension.
%Meanwhile, we have made certain modifications to its code, that is, before the data enters the model, we discretize the data to achieve better results for \textsf{Holoclean}.
(2) Yes, \textsf{Holoclean} is indeed not a time series cleaning method, but is proposed for relational data.
So we convert time series to relational data, treating timestamps and the names of each dimension as attributes and the values of each dimension as cells.
We also convert the speed constraint of each dimension to the form of a denial constraint and add the parser module into the source code.
%To achieve better results, we also quantize the continuous values of the time series into discrete values and add the parser module as well.
We quantize the continuous values of the time series into discrete values and add the parser module as well.

%(3) As mentioned in the first paragraph of this reply, \textsf{SCREEN} and \textsf{SpeedAcc} were chosen to verify the validity of the minimum fix principle, and \textsf{HTD} is also based on speed constraint and designed for multivariate data.
%\textsf{LsGreedy} is a statistical SOTA method.
%Due to borrowing the idea of smoothing in selecting repair values, this paper also incorporates the classic \textsf{EWMA} algorithm.
%We chose \textsf{Holoclean}, \textsf{CAE-M}, and \textsf{TranAD} in the hope that our algorithm can be compared with machine learning and deep learning methods.
(3) As suggested, we add a discussion in Section \ref{sect:baseline} on how and why the baselines are selected: 
\textsf{SCREEN} and \textsf{SpeedAcc} use the univariate speed constraint and follow the widely used minimum change principle.
They are selected to verify the validity of the proposed minimum fix principle.
\textsf{HTD} calculates the correlation between the dimensions and performs data cleaning over multivariate time series based on speed constraint.
\textsf{RCSWS} aims to clean GPS data and can only implement on two-dimensional data.
\textsf{LsGreedy} is a statistical SOTA method that has good accuracy.
Due to the inspiration from interpolation in choosing repair solution, we also choose the classical smoothing-based \textsf{EWMA} method as a baseline.
\textsf{Holoclean} is a representative of the machine learning method, but it is proposed for relational data.
We thus convert time series to relational data, treating timestamps and the names of each dimension as attributes and the values of each dimension as cells.
We also convert the speed constraint of each dimension to the form of a denial constraint (which can be recognized by \textsf{HoloClean}) and add the parser module into the source code.
%We find that there are few works that use deep leaning techniques for time series cleaning. 
%Therefore, we select two SOTA anomaly detection methods, \textsf{TranAD} and \textsf{CAE-M}, and consider their predicted/reconstructed values as repair candidates.
\end{reply}

\begin{question}[D1]
D1: Presentation should be improved to provide more justification of choices, and methodology details and intuition. Some of the math details can be moved to a technical/extended version. 
\end{question}

\begin{reply}
We move the math proofs to a technical version to leave more space for providing more justifications as suggested.
\end{reply}


%----------------------------------
\section*{To Reviewer 2}
Thank you very much for reading our paper carefully and your comments. 
Below is our response to your comments.
%{Accept}

\begin{question}[O1]
O1: Some sentences stating the ``triviality of a point'' are useless, in my opinion.
For example, line 635: ``The reasons of Action 1 and Action 4 are obvious.'', then why explaining it after.
\end{question}

\begin{reply}
We remove the redundant expressions in the revised version as suggested.
For example, we remove the following two paragraphs after ``The reasons of Action 1 and Action 4 are obvious.''
\end{reply}

\begin{question}[C1\& O2]
C1: A small section is then dedicated to adaptive setting of speed constraints.
While interesting, this section feels a little rushed without a proper algorithm proposed for \textsf{MTCSC-A}.

O2: Adaptive speed constraint section is a little less detailed (cf. summary).
It could be interesting to link it to the previous algorithms and/or provide a dedicated algorithm.
\end{question}

\begin{reply}
We apologize for using the same term ``window size'' for two different variables in this paper, which can lead to confusion.
In the revised version, we change w (the window size of adaptive speed) to m (monitoring interval).
%We provide the dedicated algorithm, i.e. Algorithm 5: \textsf{MTCSC-A}($\boldsymbol{\mathit{x}}, \mathit{s}$, $\mathit{b}$, $\tau$, $\mathit{m}$, $\beta$), in Section \ref{sect:adaptive-speed} to show the procedure of the adaptive method.
%The time complexity is $O(\mathit{m}+\mathit{b})+O(\mathit{w}^{2}n)$, where $m$ is the adaptive speed monitoring interval, $b$ is the bucket number, $w$ is the point window size, and $n$ is the length of the time series.
We provide the dedicated algorithm, i.e. Algorithm \ref{alg:adaptive}: \textsf{AdaptiveSpeed}($\boldsymbol{\mathit{x}}_p, \boldsymbol{\mathit{x}}_k, \mathit{s}$, $\mathit{b}$, $\tau$, $\mathit{m}$, $\beta$, $\mathit{W}_1$, $\mathit{W}_2$), in Section \ref{sect:adaptive-speed} to show the core procedure of the online cleaning method \textsf{MTCST-A} with adaptive speed.
The time complexity of Algorithm \ref{alg:adaptive} is $O(\mathit{D}+\mathit{b}+\mathit{m})$. 
\textsf{MTCSC-A} is formed by inserting Algorithm \ref{alg:adaptive} through ``$\mathit{s}$ = \textsf{AdaptiveSpeed}($\boldsymbol{\mathit{x}}_{k-1}, \boldsymbol{\mathit{x}}_k, \mathit{s}$, $\mathit{b}$, $\tau$, $\mathit{m}$, $\beta$, $\mathit{W}_1$, $\mathit{W}_2$)'' between the 3rd and 4th lines of Algorithm \ref{alg:cluster}.
Overall, the time complexity of \textsf{MTCSC-A} is $O((\mathit{D}+\mathit{b}+\mathit{m}+\mathit{w}^{2}D+2D)*n)$, where $m$ is the monitoring interval, $b$ is the bucket number, $w$ is the point window size, and $n$ is the length of the time series.

There is a typo in our algorithm \ref{alg:cluster}.
A judgment condition should be added before line 10, i.e. ``if !(\textsf{satisfy}$(\boldsymbol{\mathit{x}}_{k-1}', \boldsymbol{\mathit{x}}_{k})$ and \textsf{satisfy}$(\boldsymbol{\mathit{x}}_{k}, \boldsymbol{\mathit{x}}_{i})$)'' to prevent excessive repair of correct data.
\end{reply}

\begin{question}[O3]
O3: The comparison between results in the experiment section do not include results of statistical tests.
However, when authors affirm that their approach is more efficient than another, providing tests results could confirm the statistical significance of their allegations, this could strengthen the confidence in the authors results. 
\end{question}

\begin{reply}
Yes, in the previous paper, we did not provide statistical tests since apart from the ``separate error pattern'' (shown in Figures \ref{exp:drate-separate} and \ref{exp:size-separate}), \textsf{MTCSC} achieves better results than others (including \textsf{MTCSC-Uni}).
But as suggested, a statistical test will definitely strengthen the confidence in the results.
Therefore, we add statistical tests for different error patterns in Section \ref{sect:error-pattern} to show better differences between all methods and discuss when to use \textsf{MTCSC} or the uni version.
\end{reply}

\begin{question}[O4]
O4: In my opinion example \ref{example:repair-via-cluster} is a little too detailed and can be reduced if space needs to be saved for a revision. 
\end{question}

\begin{reply}
As suggested, we reduce example \ref{example:repair-via-cluster} by removing concrete descriptions of $\boldsymbol{\mathit{x}}_5$ to $\boldsymbol{\mathit{x}}_7$ to leave more space.
\end{reply}

\begin{question}[D1]
D1: It is great to have the source code, datasets and results.
However, the readme did not explain basic things such as the location of the source code and how to run it.
Even if it can seem pretty straightforward, to my opinion it is always a good idea to include them `just in case'.
\end{question}

\begin{reply}
We apologize for the unclear documentation. 
We provide a more detailed introduction to the source code, 
including where to find the test file, how to run the experimental tests and how to locate the corresponding datasets.
\end{reply}

%\vspace{-1em}

%----------------------------------
\section*{To Reviewer 4}
Thank you very much for reading our paper carefully and your comments.
Below is our response to your comments.
%{Accept with Shepherding}

\begin{question}[O1]
O1: In section 1.2, the authors raised 3 challenges.
It would be wonderful if they revisited them in section 5.6 to discuss what has been solved using the suggested algorithm and what is still open for future work.  
\end{question}

\begin{reply}
We revisit and discuss the effect of the proposed \textsf{MTCSC} on the 3 challenges in Section \ref{sect:highlight} as suggested.
\end{reply}

\begin{question}[O2]
O2: The implementation of an error guarantee for the adaptive speed version w.r.t. to the parameters b, theta, w, and beta would enhance the practicality of the algorithm.
\end{question}

\begin{reply}
As shown in formulas (\ref{equation:global}) and (\ref{equation:local}), our work aims to minimize the number of points changed from the original time series
However, similar to the statements in Section \ref{sect:stream}, we do not have a theoretical upper bound for \textsf{MTCSC-A} compared to \textsf{MTCSC-C}.
Fortunately, while we cannot provide an error guarantee for these parameters, we can still provide some guidelines, which are shown in Section \ref{sect:adaptive-speed}.
Nevertheless, adaptively adjusting these parameters will enhance the practicality of our proposed algorithm, which we will investigate in future work.
\end{reply}

\begin{question}[O3]
O3: Figure 8-11 used ILD-TAO, except for Figure 9, which was ECG-TAO.
Are there any specific reasons?
\end{question}

\begin{reply}
(1) To investigate the effectiveness of the proposed method in high dimensions, we perform experiments on ECG with 32 attributes.
However, the running time over the data size is quite large for all methods, so we only show the results on ECG varying error rates (Figure \ref{exp:drate-together}).
(2) We want to discuss the performance in the `separate' pattern, so we vary the error rates and data sizes on the same datasets, i.e. ILD-TAO, in Figures \ref{exp:drate-separate} and \ref{exp:size-separate}.
(3) Same datasets ILD-TAO are also used to compare the effects of different patterns, in Figures \ref{exp:size-separate} and \ref{exp:size-together}.
\end{reply}


\begin{question}[O4]
O4: According to the results, there was no clear winner.
It would be nice to have a better understanding on which data series to use the \textsf{MTCSC} or the uni version of it for example.
\end{question}

\begin{reply}
In fact, apart from the ``separate error pattern'' (shown in Figures \ref{exp:drate-separate} and \ref{exp:size-separate}), \textsf{MTCSC} achieves better results than others (including \textsf{MTCSC-Uni}).
To better illustrate the differences between all methods, distinguish them more clearly and discuss when to use \textsf{MSTCS} or the uni version, we add statistical tests for different error patterns in Section \ref{sect:error-pattern}.
%
%In addition, we recommend using \textsf{MTCSC} in the general case, as it achieves a better trade-off between efficiency and effectiveness.
We also add the recommendation for the use of \textsf{MTCSC} in the general case, as it achieves a better trade-off between efficiency and effectiveness, in Section \ref{sect:highlight}.
\end{reply}

\begin{question}[O5]
O5: Another interesting aspect would be how the algorithms are scaling with the number of dimensions.
\end{question}

\begin{reply}
%As stated in Section \ref{sect:constraint}, the distance between data points and the speed constraint in this paper are all defined in multivariate cases. 
%Therefore, our proposed \textsf{MTCSC} can clean up multivariate time series.
%Specifically,Figure \ref{exp:drate-together} shows the results on ECG with 32 dimensions.
%We find that the proposed \textsf{MTCSC} outperforms other methods and is also better than the Uni version.
%
%Although the time required to calculate the distance is slightly larger for a large number of dimensions is slightly larger, it is still applicable.
%As shown in Figure \ref{exp:drate-together}(d), \textsf{MTCSC} finishes in about 10 ms, just a bit slower than its Uni version.

%However, the relationship between the different dimensions is not trivial.
%Therefore, we did not conduct an experiment varying the data dimensions in this paper, as it is difficult to know the factors that influence performance.
Each dimension of a multivariate time series has its own characteristic. 
We cannot simply extract the information from the results of varying dimensions and distinguish the effects of performance caused by our error injection pattern, the relationship between different dimensions, or the limitation of methods.
However, in order to investigate how the algorithms are scaling with the number of dimensions and give more clearer insights, we add an experiment in Section \ref{sect:exp-dimension} under the "together" pattern over all the proposed methods (\textsf{MTCSC-G}, \textsf{MTCSC-L} and \textsf{MTCSC-C}) and analyze the results of varying dimensions.
\end{reply}

\begin{question}[O6]
O6: The outcomes depicted in Figure 14 are solely derived from datasets with only a single dimension according to Table 2.
\end{question}

\begin{reply}
We add the classification and clustering experiments on multivariate time series AtrialFib and SWJ, referring to 
``Wu, H., Hu, T., Liu, Y., Zhou, H., Wang, J. and Long, M., 2022, September. Timesnet: Temporal 2d-variation modeling for general time series analysis. (ICLR2022)''.
\end{reply}

\begin{question}[D1]
D1: The source code is not available, but the data and jar files are available. 
There is insufficient documentation to be able to conduct the experiments.
\end{question}

\begin{reply}
We apologize for the unclear documentation. 
We provide a more detailed introduction to the source code, 
including where to find the test file, how to run the experimental tests and how to locate the corresponding datasets.
\end{reply}


